Variation Spaces for Multi-Output Neural Networks: Insights on Multi-Task Learning and Network Compression

This paper introduces a novel theoretical framework for the analysis of vector-valued neural networks through the development of vector-valued variation spaces, a new class of reproducing kernel Banach spaces. These spaces emerge from studying the regularization effect of weight decay in training networks with activations like the rectified linear unit (ReLU). This framework offers a deeper understanding of multi-output networks and their function-space characteristics. A key contribution of this work is the development of a representer theorem for the vector-valued variation spaces. This representer theorem establishes that shallow vector-valued neural networks are the solutions to data-fitting problems over these infinite-dimensional spaces, where the network widths are bounded by the square of the number of training data. This observation reveals that the norm associated with these vector-valued variation spaces encourages the learning of features that are useful for multiple tasks, shedding new light on multi-task learning with neural networks. Finally, this paper develops a connection between weight-decay regularization and the multi-task lasso problem. This connection leads to novel bounds for layer widths in deep networks that depend on the intrinsic dimensions of the training data representations. This insight not only deepens the understanding of the deep network architectural requirements, but also yields a simple convex optimization method for deep neural network compression. The performance of this compression procedure is evaluated on various architectures.

==> sections/perturbation_arg.tex <==
% \section{Perturbation Argument}
% \def\by{{\boldsymbol{y}}}
% \joe{Could we just use general lipschitz loss?}



% Consider a two output case.  Denote the two output sequences we are fitting by $\by_1$ and $\by_2$, and let $\widehat \by_1$ and $\widehat \by_2$ denote the output of a neural network fit to these data.  Specifically, $\widehat \by_1 = \sum_i v_{i,1} \vec{\phi}_i$ and $\widehat \by_2 = \sum_i v_{i,2} \vec{\phi}_i$, where $\vec{\phi}_i$ denotes the $i$th ReLU neuron evaluated on the input data points.    The objective value of this network is
% $$ \mathcal{L}(y_i, f(\vec{x}_i)) + \lambda \norm{f}_{\V(\R^d)}, \quad \lambda > 0$$

% This fit has an objective value of
% $$\|\by_1 -\widehat\by_1\|_2^2 + \|\by_2 -\widehat\by_2\|_2^2 \ + \ \lambda \times \mbox{VV-norm of network}$$
% Now suppose that there exists two neurons, say $j$ and $k$, such that $v_{j,1},v_{k,2}\neq 0$ and $v_{k,1}=v_{j,2}=0$ (i.e., $j$ contributes only to the first output and $k$ only contributes to the second output) and that 
% $\|\vec{\phi}_j-\vec{\phi}_k\|_2\leq \epsilon$.  Consider replacing neuron $\vec{\phi}_{k}$ with neuron $\vec{\phi}_{j}$, so that the two outputs ``share" $\vec{\phi}_{j}$ and define
% $$\tilde\by_2 = \sum_{i\neq k} v_{i,2} \vec{\phi}_{i} + v_{k,2} \vec{\phi}_{j} \ . $$
% Using $\tilde\by_2$ instead of $\widehat\by_2$ may have a slightly larger squared error, but will have a smaller VV-norm contribution.

% The difference in the objective values using $\widehat\by_2$ and $\tilde\by_2$ is given by
% \begin{eqnarray*}
%    \|\by_2 -\tilde\by_2\|_2^2-\|\by_2 -\widehat\by_2\|_2^2 + \lambda \big((v_{j,1}^2+v_{k,2}^2)^{1/2} -(|v_{j,1}|+|v_{k,2}|)\big)
% \end{eqnarray*}
% since all other terms in the VV-norms are equivalent.  We can bound the squared error difference as follows.  Note that $\|\widehat\by_2 -\tilde\by_2\|_2<|v_{k,2}|\epsilon$ and so
% \begin{eqnarray*}
%    \|\by_2 -\tilde\by_2\|_2^2-\|\by_2 -\widehat\by_2\|_2^2 & \leq & \|\by_2 -\widehat\by_2 + \widehat\by_2 -\tilde\by_2\|_2^2-\|\by_2 -\widehat\by_2\|_2^2 \\
%    & \leq & (\|\by_2 -\widehat\by_2\|_2 + \|\widehat\by_2 -\tilde\by_2\|_2)^2-\|\by_2 -\widehat\by_2\|_2^2 \\
%    & = & 2\|\by_2 -\widehat\by_2\|_2  \|\widehat\by_2 -\tilde\by_2\|_2 + \|\widehat\by_2 -\tilde\by_2\|_2^2 \\
%    & \leq & 2\epsilon |v_{k,2}|\|\by_2 -\widehat\by_2\|_2  + \epsilon^2|v_{k,2}|^2 
% \end{eqnarray*}
% \rob{if we assume an additive (over examples) L-Lip loss function instead, then the difference in losses is
% $$L(\tilde\by_2)-L(\widehat\by_2) \ \leq \ L \|\widetilde\by_2-\widehat\by_2\|$$
% for some norm (we could take it to be L1 and then assume $\|\phi_{j,1}-\phi_{j,2}\|_1\leq \epsilon$).  Hence, the differences of losses would be bounded by $L\epsilon  |v_{j,1}| \, |1-\alpha|$.  }
% The difference of the VV-norms is
% $$\lambda|v_{k,2}| (\sqrt{1+\alpha^2}-(1+\alpha))$$
% where $\alpha = |v_{j,1}/v_{k,2}|$.
% This is always negative (assuming $|v_{k,2}|>0$) and tends to $-\lambda|v_{k,2}|$ as $\alpha$ increases.  Putting this all together, the the objective value using $\tilde\by_2$ is smaller than the objective value using $\widehat\by_2$ if
% $$\lambda|v_{k,2}| (\sqrt{1+\alpha^2}-(1+\alpha)) \ > \ 2\epsilon |v_{k,2}| \|\by_2 -\widehat\by_2\|_2  + \epsilon^2 |v_{k,2}|^2 \ , $$
% which clearly holds for sufficiently small $\epsilon$.






% Consider a two output case.  Denote the two output sequences we are fitting by $\by_1$ and $\by_2$, and let $\widehat \by_1$ and $\widehat \by_2$ denote the output of a neural network fit to these data.  Specifically, $\widehat \by_1 = \sum_i v_{i,1} \vec{\phi}_{i,1}$ and $\widehat \by_2 = \sum_i v_{i,2} \vec{\phi}_{i,2}$, where $\vec{\phi}_{i,j}$ denotes the $i,j$th ReLU neuron evaluated on the input data points.  The number of terms in the sums need not be the same.  The objective value of this network is
% $$ \mathcal{L}(y_i, f(\vec{x}_i)) + \lambda \norm{f}_{\V(\R^d)}, \quad \lambda > 0$$

% This fit has an objective value of
% $$\|\by_1 -\widehat\by_1\|_2^2 + \|\by_2 -\widehat\by_2\|_2^2 \ + \ \lambda \times \mbox{VV-norm of network}$$
% Now suppose that there exists two neurons, one contributing to output 1 and another to output 2, that are close to each other.  Without loss of generality, say $\vec{\phi}_{j,1}$ and $\vec{\phi}_{j,2}$ are different but close in the sense that $\|\vec{\phi}_{j,1}-\vec{\phi}_{j,2}\|_2\leq \epsilon$, and assume that these two are distinct from all other neurons in the network.  Moreover, assume that $|v_{j,2}| = \alpha |v_{j,1}|$ for some $\alpha >0$.  Consider replacing neuron $\vec{\phi}_{j,2}$ with neuron $\vec{\phi}_{j,1}$, so that the two outputs ``share" $\vec{\phi}_{j,1}$ and define
% $$\tilde\by_2 = \sum_{i\neq j} v_{i,2} \vec{\phi}_{i,2} + v_{j,2} \vec{\phi}_{j,1} \ . $$
% Using $\tilde\by_2$ instead of $\widehat\by_2$ may have a slightly larger squared error, but will have a smaller VV-norm contribution.



% Consider a two output case.  Denote the two output sequences we are fitting by $\by_1$ and $\by_2$, and let $\widehat \by_1$ and $\widehat \by_2$ denote the output of a neural network fit to these data.  Specifically, $\widehat \by_1 = \sum_i v_{i,1} \phi_{i,1}$ and $\widehat \by_2 = \sum_i v_{i,1} \phi_{i,1}$, where $\phi_{i,j}$ denotes a ReLU evaluated on the input data points.  The number of terms in the sums need not be the same.  This fit has an objective value of
% $$\|\by_1 -\widehat\by_1\|_2^2 + \|\by_2 -\widehat\by_2\|_2^2 \ + \ \lambda \times \mbox{VV-norm of network}$$
% Now suppose that there exists two neurons, one contributing to output 1 and another to output 2, that are close to each other.  Without loss of generality, say $\phi_{j,1}$ and $\phi_{j,2}$ are different but close in the sense that $\|\phi_{j,1}-\phi_{j,2}\|_2\leq \epsilon$, and assume that these two are distinct from all other neurons in the network.  Moreover, assume that $|v_{j,2}| = \alpha |v_{j,1}|$ for some $\alpha >0$.  Consider replacing neuron $\phi_{j,2}$ with neuron $\phi_{j,1}$, so that the two outputs ``share" $\phi_{j,1}$ and define
% $$\tilde\by_2 = \sum_{i\neq j} v_{i,2} \phi_{i,2} + v_{j,2} \phi_{j,1} \ . $$
% Using $\tilde\by_2$ instead of $\widehat\by_2$ may have a slightly larger squared error, but will have a smaller VV-norm contribution.
% The difference in the objective values using $\widehat\by_2$ and $\tilde\by_2$ is given by
% \begin{eqnarray*}
%    \|\by_2 -\tilde\by_2\|_2^2-\|\by_2 -\widehat\by_2\|_2^2 + \lambda \big((v_{j,1}^2+v_{j,2}^2)^{1/2} -(|v_{j,1}|+|v_{j,2}|)\big)
% \end{eqnarray*}
% since all other terms in the VV-norms are equivalent.  We can bound the squared error difference as follows.
% \begin{eqnarray*}
%    \|\by_2 -\tilde\by_2\|_2^2-\|\by_2 -\widehat\by_2\|_2^2 & \leq & \|\by_2 -\widehat\by_2 + \widehat\by_2 -\tilde\by_2\|_2^2-\|\by_2 -\widehat\by_2\|_2^2 \\
%    & \leq & (\|\by_2 -\widehat\by_2\|_2 + \|\widehat\by_2 -\tilde\by_2\|_2)^2-\|\by_2 -\widehat\by_2\|_2^2 \\
%    & = & 2\|\by_2 -\widehat\by_2\|_2  \|\widehat\by_2 -\tilde\by_2\|_2 + \|\widehat\by_2 -\tilde\by_2\|_2^2 \\
%    & \leq & 2\epsilon \|\by_2 -\widehat\by_2\|_2  + \epsilon^2|v_{j,1}-v_{j,2}|^2 \\
%    & = & 2\epsilon \|\by_2 -\widehat\by_2\|_2  + \epsilon^2 |v_{j,1}| \, |1-\alpha|
% \end{eqnarray*}
% \rob{if we assume an additive (over examples) L-Lip loss function instead, then the difference in losses is
% $$L(\tilde\by_2)-L(\widehat\by_2) \ \leq \ L \|\widetilde\by_2-\widehat\by_2\|$$
% for some norm (we could take it to be L1 and then assume $\|\phi_{j,1}-\phi_{j,2}\|_1\leq \epsilon$).  Hence, the differences of losses would be bounded by $L\epsilon  |v_{j,1}| \, |1-\alpha|$.  }
% The difference of the VV-norms is
% $$\lambda|v_{j,1}| (\sqrt{1+\alpha^2}-(1+\alpha))$$
% This is always negative (assuming $|v_{j,1}|>0$) and tends to $-\lambda|v_{j,1}|$ as $\alpha$ increases.  Putting this all together, the the objective value using $\tilde\by_2$ is smaller than the objective value using $\widehat\by_2$ if
% $$\lambda|v_{j,1}| (\sqrt{1+\alpha^2}-(1+\alpha)) \ > \ 2\epsilon \|\by_2 -\widehat\by_2\|_2  + \epsilon^2 |v_{j,1}| \, |1-\alpha| \ , $$
% which clearly holds for sufficiently small $\epsilon$ and fixed values for $\lambda$ and $\alpha$.


